Reduction of laser intensity noise over 1 MHz band for single atom trapping

We reduce the intensity noise of laser light by using an electro-optic modulator and a cousto-optic modulator in series. The electro-optic modulator reduces noise at high frequency(10 kHz to 1 MHz), while the acousto-optic modulator sets the average power of the light and reduces noise at low frequency (up to 10 kHz). The light is then used to trap single sodium atoms in an optical tweezer, where the lifetime of the atoms is limited by parametric heating due to laser noise at twice the trapping frequency. With our noise eater, the noise is reduced by up to 15 dB at these frequencies, and the lifetime is increased by an order of magnitude to around 6 seconds. Our technique is general and acts directly on the laser beam, expanding laser options for sensitive optical trapping applications.

==> Old/latexmkrc <==
## Sometimes when the references is very near the end of a page/column, latexmk fails to recognise when bibtex needs to be run. This rule forces bibtex to be run everytime.
$pdflatex = 'pdflatex --shell-escape %O %S; bibtex %R';



###############################
# Post processing of pdf file #
###############################

# assume the jobname is 'output' for Overleaf v2
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    my $QPDF = "/usr/bin/qpdf";
    return if ! -x $QPDF; # check that qpdf exists
    my $status = system($QPDF, "--linearize", "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
	system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
        $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
	system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
	if (-e $rtex_file) {
		do_knitr($rtex_file);
	}
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
	# change directory for a limited scope
	my $orig_dir = cwd();
	my $subdir = dirname($target);
	chdir($subdir);
	# run chktex on main file
	$status = system(
    "/usr/bin/run-chktex.sh",
    $orig_dir,
    $file
  );
	# go back to original directory
	chdir($orig_dir);

	# in VALIDATE mode we always exit after running chktex
	# otherwise we exit if EXIT_ON_ERROR is set

	if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
	    # chktex doesn't let us access the error info via exit status
	    # so look through the output
	    open(my $fh, "<", "output.chktex");
	    my $errors = 0;
	    {
		local $/ = "\n";
		while(<$fh>) {
		    if (/^\S+:\d+:\d+: Error:/) {
			$errors++;
			print;
		    }
		}
	    }
	    close($fh);
	    exit(1) if $errors > 0;
	    exit(0) if $ENV{'CHKTEX_VALIDATE'};
	}
    }
}

==> Old/scrap.tex <==
%\subsection{Draft Abstract, technique motivated}
%We developed a servo system with high-bandwidth intensity noise reduction for lasers. Up to $\SI{18}{\decibel}$ noise attenuation is achieved in the $\SI{100}{\kilo\hertz}$--$\SI{1}{\mega\hertz}$ region and the servo-ed laser provides us an optical tweezer where a single sodium atom has a lifetime of about 5 seconds, which is 10 times longer than the free-running condition. The stable, long-term trapping atoms could servo as a great platform for quantum computation and information. The servo design can be used for intensity noise reduction of any available wavelength and power, allowing coherent motional control of neural atoms, molecules and ions in general.
%\subsection{Draft Abstract, physics motivated}
%(maybe use in conclusion) Optical trapped neutral atoms and molecules have provided an attractive platform for quantum many-body physics, quantum information and computation. For those application, robust coherent quantum state is a crucial prerequisite. Coherent transfer is highly sensitive to the motional ground state occupancy of the individual atoms and requires long (> $\SI{1}{\second}$) trap lifetimes. Therefore, we developed a servo system which suppressed the intensity noise in a high bandwidth up to $\SI{1}{\mega\hertz}$, and obtained a stabilized optical trap where the trapped sodium atom has a lifetime of about 5 seconds.
% \textcolor{blue}{Eliot: I'm just writing random stuff to see what comes out}\\
%\textcolor{blue}{..................................................}\\

%For several decades, people have been using lasers. Lasers are great because they are stable both in frequency and intensity. There's a lot of applications for lasers, and most of them require some level of intensity stability, especially surrounding the frequencies relevant to the system of study. Some systems even require both DC control and low noise at frequencies higher than 100 kHz. Many lasers have integrated, internal noise eaters, but it can be helpful to have a general, external method for reducing noise when there are technological, practical, or financial limitations on the type of laser system you can buy.

%Our lab specifically uses lasers to form optical tweezers. Tweezers are super useful and have been demonstrated in several atomic species, and even molecular species (soon to be us!). However, to generalize tweezers for more species, we'll need stable light sources at a bunch of different frequencies. Furthermore, if you want an array of tweezers (as many labs do), you'll need a lot of power. This can prove limiting because it's possible there's not a clean, high-power laser source at the wavelength you need. 

%Our lab specifically is interested in developing an array of sodium tweezers for quantum chemistry and simulation reasons. Sodium tweezers need to be between 620 and 700 nm because of the AC Stark shift. However, we need like 3 W directly out of the laser per trap, and it's hard to find a direct laser source for that. We're therefore trying an SFG setup to produce the light. One of our input lasers happens to be noisy, which leads to noise on the output as well. The relevant requencies for our experiment is the shot-to-shot frequency (~3 Hz) and the parametric heating frequency (~500 kHz). Therefore, we need low noise at both DC (<10 Hz) and high frequency (200 kHz~1 MHz). This produces a major challenge, as we couldn't find any external noise eaters that work for DC-1 MHz.

%Our ingenious idea is to use two different servo systems to independently control high- and low- frequency noise.

%\textcolor{blue}{..................................................}\\
%\textcolor{blue}{Random stuff over}\\

%\textcolor{green}{~Something about lasers.~} 

%Lasers have become an important tool in a wide range of science and engineering fields due to their tight confinement of light and high frequency and intensity stability. 


%\textcolor{blue}{break}

%Optical tweezers have emerged as a powerful approach to a variety of applications in quantum simulation, quantum information, and quantum chemistry\cite{bernien2017probing,yu2019scalable,Liu900,PhysRevLett.120.113602} (pick better references). \textcolor{red}{I could add more general information here and put a paragraph break before moving on to our experiment} In our lab, we use tweezers to trap individual sodium and cesium atoms and combine them to coherently form NaCs molecules [cite]. Coherent transfer is highly sensitive to the motional ground state occupancy of the individual atoms and requires long (> $\SI{1}{\second}$) trap lifetimes. \textcolor{red}{Therefore, to achieve high transfer efficiency, we must limit heating of the atoms trapped in the tweezers}. The major heating mechanism in our system is parametric heating due to laser intensity fluctuations of the tweezer beams. Intensity noise at twice the harmonic trapping frequency is especially \textcolor{red}{damaging}, as it induces transitions between harmonic oscillator states in the trap \cite{PhysRevA.56.R1095}. For typical trap depths of a few $\si{\milli\kelvin}$, this means controlling intensity noise in the $\SI{100}{\kilo\hertz}$--$\SI{1}{\mega\hertz}$ band.


%   \cite{levine2019parallel,kaufman2012cooling}and .(TODO - maybe SNR?) of the experiments.....

 %However, most commercial laser noise eaters only work in a lower frequency region. Early approaches\cite{harb1994suppression, Taccheo:00} for intensity noise reduction directly fed back on the laser current, which is not possible for all laser drivers. More recently, a light source with suppressed intensity noise\cite{blatt2015low} has been used for optical lattices to get stable trapping with long lifetimes. 

%Here, we develop a servo system with high-bandwidth intensity noise reduction by combining an electro-optic modulator (EOM) servo and an acousto-optic modulator (AOM) servo to independently deal with high  ($\SI{100}{\kilo\hertz}$--$\SI{1}{\mega\hertz}$) and low (DC--$\SI{100}{\kilo\hertz}$) frequency noise. Up to $\SI{18}{\decibel}$ noise attenuation is achieved in the $\SI{100}{\kilo\hertz}$--$\SI{1}{\mega\hertz}$ region and up to $\SI{10}{\decibel}$ in the $1\si{\kilo\hertz}$--$\SI{100}{\kilo\hertz}$ region. With the servo system we developed, we can trap a single sodium atom for longer than $\SI{5}{\second}$, which provides a stable platform for various applications(TO cite). By suppressing parametric heating in our optical tweezer, we achieve a lifetime about 10 times longer than the free-running condition.(\textcolor{red}{if we find a pi, we will add a sentence here to show off our theory and experiment matches well}

%A fundamental prerequisite for laser sources suitable for optical dipole trapping is the occurrence \textcolor{blue}{(word choice)} of low relative intensity noise. Since the typical depth of optical dipole trap is a few $\si{\milli\kelvin}$ and the trap frequency is proportional to the square root of trap depth, the trap frequency is usually located in $100\si{\kilo}$--$\SI{1}{\mega\hertz}$, while commercial laser noise eater only works in a much lower frequency region(TODO). Due to the parametric heating mechanism, noise in this frequency region will greatly reduce the lifetime of an atom. This circumstance may strongly affect the lifetime of the atom trapped in the tweezer. This problem becomes a major constraint for quantum simulation or quantum computation applications which call for long coherence time.
%\textcolor{red}{An Eliot rewrite of the previous paragraph:}

%To get stable optical dipole traps with enough depth, 
%\textcolor{red}{experiment setup}

% \textcolor{blue}{.....................}
%  We generate $\SI{671}{\nano\meter}$ light with a sum-frequency generation (SFG) setup. We use a nonlinear crystal to combine $\SI{1557}{\nano\meter}$ light from an NKT photonics erbium-doped fiber laser with $\SI{1178}{\nano\meter}$ light from an MPB Raman fiber amplifier to get about $\SI{600}{\milli \watt}$ of $\SI{671}{\nano\meter}$ light. The intensity noise on the $\SI{671}{\nano\meter}$ light mainly comes from the $\SI{1178}{\nano\meter}$ laser and nonlinear effects of the crystal.
 
 %(VRFA-P-2000-589-SF)
 
 %\subsection{High-frequency servo}
%Our system setup is shown in Fig. \ref{fig:setup}. The $\SI{671}{\nano\meter}$ light exits the SFG crystal. We use a quarter waveplate and a half waveplate to modulate the polarization of the beam before entering the EOM so that about $80 \%$ the power transmits through the polarizing beam splitter (PBS). In this way, we get a balance of high power and best intensity noise reduction. We use a beam sampler to pick up about $1\%$ of the transmitted beam by the PBS after the EOM. One of the reflected beam from the sampler is for servoing and the other one is for monitoring. The beam for servoing is picked up by a $\SI{150}{\mega\hertz}$ bandwidth PDA10A photodiode and processed by a homemade proportional-integral-derivative (PID) circuit. A PDA36A photodiode with a bandwidth of $\SI{10}{\mega\hertz}$ bandwidth is used to monitor the noise spectrum. Both the feedback and monitoring photodiodes are placed on the transmission port of the PBS, as the reflection port has a different intensity noise spectrum.

% To maximize the noise reduction of the servo, the beam is focused by a plano-convex lens with a $\SI{75}{\milli\meter}$ focal length to the center of the active area of the servoing photodiode. In order to separate frequency regions, a bias tee is placed right after the photodiode so that the circuit only feeds back the high-frequency signal. The bias tee in our setup is homemade with a $\SI{3}{\decibel}$ attenuation cutoff at $\SI{17}{\kilo\hertz}$. It filters signals below the cutoff frequency without changing the phase or amplitude of the signal above the cutoff. Both the DC end of the bias tee and the setpoint of the PID circuit are terminated with standard $\SI{50}{\ohm}$ terminators. In the experiment, we use a combination of proportional and derivative control to minimize the noise in the high frequency region while keeping the bandwidth as large as possible. Since the maximum output signal of the PID circuit is relatively small, we add a homemade amplifier before the EOM to effectively increase the gain of the PID circuit. Two crucial points about the design of the amplifier are high gain and zero phase lag over a high bandwidth up to $\SI{1}{\mega\hertz}$. The high gain needs to match the halfwave voltage of the EOM so that the polarization of the light could be efficiently regulated. The zero phase lag will ensure the high bandwidth of the EOM servo. The open-loop transfer function of the PID together with the homemade amplifier is shown in Fig.\ref{fig:tf} for reference. It shows that in the high frequency region, it has a higher gain than in the low frequency region and a negative phase which effectively feed back to the loop.  

% Considered the phase delay in EOM and the optical path, the EOM servo system is a controlled object with inertia, and we need to improve the dynamic characteristics of the system adjustment process. \textcolor{red}{(This previous sentence is confusing. Not really sure what you mean here.)} In order to avoid the possible oscillation and even destabilization during the adjustment of the error, we want to have a phase-lead compensator, which is generated by a combination of proportional and derivative feedback. The circuit we are using have two proportional control, two integral control and one derivative control. \textcolor{red}{We should talk about this paragraph.}
 
 
%\textcolor{red}{*}After the circuit, we add another homemade electric amplifier to the output of the servo and connect it to the EOM. 
%The main idea of the design of the amplifier is to match the maximum noise signal with the voltage required to produce a retardant of $\pi$ rad with a broad bandwidth. \textcolor{red}{This sentence is confusing.} The combination of the waveplate configuration is carefully designed to make sure the EOM could act on the slope of the polarization while wasting less optical power. The amplitude modulating EOM operates as a voltage dependent waveplate. There are a fast and a slow axis in the birefringent crystal whose birefringence depends on the applied voltage. It introduces a phase delay between the two axes. 

% To measure the spectra, we use a low-noise SR560 preamplifier from Stanford Research Systems to improve the signal-to-noise ratio (SNR) and measure it with a Digital Discovery field programmable gate array (FPGA) board from Digilent. The $\SI{1}{\mega\hertz}$ bandwidth of the preamplifier covers the frequency region we are interested in. Additionally, we measure the spectra above $\SI{1}{\mega\hertz}$ using a ZFL-1000LN+ amplifier from Mini-circuits. The results show that the EOM servo has no appreciable effect on the intensity noise spectrum up to $\SI{10}{\mega\hertz}$. since the SR560 preamplifier has a flatter gain in a large range which makes the measurement convenient, all spectra presented in this paper are measured with the Stanford Research Systems preamplifier.

% In Fig. \ref{fig:high_spectrum}, we show the comparison of the intensity noise spectral densities with and without the servo. The spectra are normalized to the DC power and are commonly
% referred to as relative intensity-noise (RIN) spectra. These spectra are measured on the experiment table before the vacuum chamber so that the noise of the fiber is also considered. The background is measured when the light is blocked so it is mainly caused by the dark current of the photodiode. The spectra are normalized to the DC power and are commonly referred to as relative intensity-noise (RIN) spectra \textcolor{blue}{cite}. The intensity noise is reduced by up to $\SI{18}{\decibel}$ for Fourier frequencies below $\SI{1}{\mega\hertz}$. Though the intensity noise of the free-running laser is not evenly distributed over the high-frequency region, it is almost constant when servoed, allowing stable trapping with long lifetimes in different trap depths.

% \subsection{AOM servo}
%After the EOM servo, we use an AOM servo to control the low frequencies from DC to about $\SI{100}{\kilo\hertz}$. We focus the beam into the AOM to maximize its switching bandwidth. The beam of the first diffraction order is re-collimated by another plano-convex lens with the same focal length while the zeroth order is dumped (which is not shown in the Fig.\ref{fig:setup}). The signal for the servo is picked up by a wedged beam sampler and focused onto a PDA10A2 photodiode. Here, we use the same model bias tee as in the high-frequency servo to filter out the high frequency noise. The bandwidth of the DC (low-pass) end is about $\SI{100}{\kilo\hertz}$ and the RF end is terminated with a standard $\SI{50}{\ohm}$ terminator. The DC output of the bias tee is connected to the input of the PID circuit and the DC setpoint of the PID is controlled by the experiment control computer. To reduce the steady-state error and stabilize the servo, we primarily use integral control with little proportional or derivative feedback. A $\SI{100}{\kilo\hertz}$ low-pass filter is added to the output of the circuit to ensure that no high-frequency electronic noise is written onto the optical intensity spectrum. We tune the PID settings so that the PID does not introduce any other resonance, especially in the high frequency region. The RF signal for driving the AOM is combined with the servo signal with the mixer ZAD-1-1+ . We set the RF signal amplitude such that the AOM transmission reaches maximum when the servo is railed. In the experiment, we change the DC power of the light by changing the setpoint of the servo, which effectively changes the RF power driving the AOM.

% The AOM servo provides DC power control and an up to $\SI{10}{\decibel}$ intensity noise suppression in a lower frequency region, as shown in Fig. \ref{fig:low_spectrum}. We measure the intensity noise spectrum when the laser is blocked (background), free-running, only EOM servo-ed (with AOM servo railed), and both AOM and EOM servo-ed. It is clear that the EOM servo doesn't add extra noise in the low frequency region and the AOM servo only slightly increases noise in the intermediate region from $\SI{10}{\kilo\hertz}$ to $\SI{100}{\kilo\hertz}$. It could be re-optimized for better performance if required and also there are commercial products dealing with this frequency region.

% Based on the spectra in the high and low frequency regions, we calculate the suppression factor of our servo system in the full frequency band in Fig.\ref{fig:suppresion}. For reference, we also label approximately twice our axial and radial trapping frequencies in the figure. From the suppression factor figure, we see an approximately $\SI{2}{\decibel}$ intensity noise reduction at twice the axial frequency and an $\SI{13}{\decibel}$reduction at twice the radial frequency of our optical tweezer.

% The $\SI{1}{\mega\hertz}$ bandwidth of the preamplifier covers the frequency region we are interested in. Additionally, we measure the spectra above $\SI{1}{\mega\hertz}$ using a ZFL-1000LN+ amplifier from Mini-circuits.
%The results show that the EOM servo has no appreciable effect on the intensity noise spectrum up to $\SI{10}{\mega\hertz}$.

. For a set of given parameter including the initial temperature and the heating rate, we could numerically solve the Fokker Planck equation and get the survival probability as a function of time. The $\chi^2$ is defined by the square of the error between the experimental data and the calculated survival probability divided by the uncertainty in the experiment:

\textcolor{blue}{..................................................}
We characterize the effect of tweezer intensity noise on the atom by measuring trap lifetimes under different servo conditions. A time plot of the experimental sequence is shown in Fig. \ref{fig:time}. Due to technical reasons (\textcolor{blue}{limited power}), we are unable to load atoms directly into our $\SI{671}{\nano\meter}$ tweezer. Instead, we load and image atoms first in a $\SI{700}{\nano\meter}$ tweezer, then transfer to the $\SI{671}{\nano\meter}$ tweezer. We then transfer back to the $\SI{700}{\nano\meter}$ tweezer for final atomic imaging. We measured the trap depth and trap frequency of the $\SI{700}{\nano\meter}$ tweezer by Raman sideband spectrum and rescale the complex polarizability for $\SI{671}{\nano\meter}$\cite{grimm2000optical}. The trap depth $U_0$ and the effective trap frequency $f_{trap}$ are: 
\begin{equation}
    \begin{split}
        U_0&=\SI{5.7}{\milli\kelvin} \\
        f_{trap}&=\SI{295}{\kilo\hertz}
    \end{split}
\end{equation}

By varying the hold time of the tweezer and observing how the survival probability varies with time, we can extract the heating rate. Lifetime measurements for the two servo conditions are shown in Fig. \ref{fig:lifetime}. For every data point, we load over 500 atoms. We find exceptionally low heating rates and correspondingly long lifetimes when the tweezer light is controlled by our intensity noise reduction system.

%\textcolor{brown}{present the extracted heating rate and compare it to the noise intensity}
We fit the survival probabilities to a curve following the procedure in \cite{gehm1998dynamics}. We assume an initial Maxwell-Boltzmann energy probability density with the temperature as a free fitting parameter since every single test we load only one atom in the tweezer and there is no exchange interaction. For a set of given parameter including the initial temperature and the heating rate, we could numerically solve the Fokker Planck equation and get the survival probability as a function of time. The $\chi^2$ is defined by the square of the error between the experimental data and the calculated survival probability divided by the uncertainty in the experiment:
\begin{equation}
    \chi^2(T_0, \Gamma_{1}, \Gamma_{2})=\sum_{i=1,2...5}\frac{(x_{1_i}-x(t_i, T_0, \Gamma_1))^2}{{\sigma_1}_i^2} + \sum_{j=1,2...7}\frac{({x_2}_j- x({t_2}_j, T_0, \Gamma_2))^2}{{\sigma_2}_j^2}
\end{equation}
The subscript 1 refers to the free-running condition and 2 for with the servo. $\Gamma_{1,2}$ is the heating rate and $T_0$ is the initial temperature of the atoms in the tweezer. The time series we measure the survival probability is donated by $t_{1,2}$, the corresponding survival probabilities are donated by $x_{1,2}$ and the uncertainty by $\sigma_{1,2}$. $x(t,T,\Gamma)$ is survival probability calculated by the numerical integral of density distribution below the trap depth where the density distribution is the numerical solution of the Fokker-Planck equation at the time $t$ with the heating rate $\Gamma$ and initial temperature $T$. The optimization process is to find a set of proper $\Gamma_{1,2}$,$T_0$ so that the $\chi^2$ is minimized. We do the optimization by a two level scan: firstly we fix the $T_0$ and scan $\Gamma_1$ and $\Gamma_2$, as the two summation terms are independent(first summation only relies on $\Gamma_1$ and the second summation only relies on $\Gamma_2$), we separately scan $\Gamma_1$ and scan $\Gamma_2$ to find a minimized $\chi^2$ with the fixed $T_0$; secondly we scan the $T_0$ to minimize $\chi^2$. We then find the global minimum of $\chi^2$ and take the corresponding parameter as the fitting results.
%We then optimize the fit of each curve by varying the heating rates. The time evolution of the distribution is described by the Fokker-Plank equation. The survival probabilities are calculated by the summation of the atoms with less energy than the trap depth. 
From the fitted curves, we calculate the initial temperature and heating rates of the system to be:
\begin{equation}
    \begin{split}
        &T_0 = \SI{0.50\pm0.02}{\milli\kelvin}\\
        &\Gamma_{1} = \SI{3.50\pm 0.03}{\second^{-1}}\\
        &\Gamma_{2} = \SI{0.348\pm 0.003}{\second^{-1}}\\
    \end{split}
\end{equation}

%where the heating rate $\Gamma$ is defined as the exponential growth rate of the average energy: 
%\begin{equation}
%    \langle \dot{E} \rangle=\Gamma E
%\end{equation}

From the relationship between heating rate and intensity noise,
\begin{equation}
\Gamma_x=\pi^2\times f_{x}^2\times S_k(2f_{tx})
\label{eq:gamma}
\end{equation}
where $S_k(2f_{x})$ is the one-sided power spectrum of the fractional fluctuation in the spring constant of the tweezer at double trap frequency in x dimension. And the effective heating rate of this system is the arithmetic mean of the heating rate of the three dimensions:

\begin{equation}
\Gamma=\frac{\Gamma_x+\Gamma_y+\Gamma_z}{3}
\label{eq:gamma_mean}
\end{equation}

In our system, we measured the trap frequency in three dimensions by TODO and got
\begin{equation}
\begin{split}
    f_{\text{radial}}&=f_x=f_y=\SI{360\pm 3}{\kilo \hertz}\\
    f_{\text{axial}}&=f_z=\SI{38\pm 1}{\kilo\hertz}\\
\end{split}
\label{eq:trap frequency}
\end{equation}
we measured the experimental heating rate for both condition(the subscribe n refers to results calculated by noise spectra):
\begin{equation}
    \begin{split}
     &\Gamma_{\text{free}} = \SI{5.1\pm0.9}{\second^{-1}}\\
     &\Gamma_{\text{servo}} = \SI{0.3\pm 0.1}{\second^{-1}}\\
    \end{split}
\end{equation}
The noise spectra results and the lifetime test on the atom are in close agreement that 10 times lifetime of the atom in the tweezer is gained by the servo system and the half-life of the sodium atom is longer than $\SI{5}{\second}$.  

We stochastically load sodium atoms from a magneto-optical trap (MOT) \cite{hutzler2017eliminating}. After turning off the MOT, we image the atoms in a 700 nm trap, in order to then post select on trials where a sodium atom is successfully loaded. We then transfer the atom to the 671 nm trap, in the servo-ed and free running condition for variable hold times. We then image again, back in the 700 nm trap, to see if the atom had been lost from the trap. The survival probability of the atom as a function of time is shown in figure \ref{fig:lifetime}. There is a clear increase in the atom lifetime when the noise eater system is used. \\

\subsection{Quantitative Analysis}
To confirm that parametric heating is indeed the mechanism for atom loss, we take a more quantitative approach. We extract heating rates from the survival data in figure \ref{fig:liftime}. Furthermore, we also compare these heating rates to the expected heating rates based on the measured intensity noise spectrum of the laser. 

\subsubsection{Heating Rate from Atom Survival}
We fit the survival probabilities following the model in \cite{gehm1998dynamics}. We assume an initial Maxwell-Boltzmann energy distribution, instead of a Bose-Einstein distribution, since we are loading atoms one at a time. We then evolve the energy distribution to time $ t $ using a Fokker-Planck equation with a heating rate, $ \Gamma $. Then, to obtain the survival of the atoms, we calculate the portion of the distribution that is lower in energy than the trap depth. From this procedure, we fit the heating rate, and the ratio of the initial temperature to the trap depth. We measure the trap power, beam waist, and convert to a trap depth using the polarizability \cite{arora2007magic}. Using this trap depth of 5.7 mK, we can then extract an initial temperature, $ T_0 $. \\
We fit both the servo-ed and free running cases shown in figure \ref{fig:lifetime} together, extracting a common $T_0$ along with heating rates, $\Gamma_{\text{servo}}$ and $ \Gamma_{\text{free}} $:

\begin{equation} \label{data_heating}
    \begin{split}
        &T_0 = \SI{0.50\pm0.02}{\milli\kelvin}\\
        &\Gamma_{\text{free}} = \SI{3.50\pm 0.03}{\second^{-1}}\\
        &\Gamma_{\text{servo}} = \SI{0.348\pm 0.003}{\second^{-1}}\\
    \end{split}
\end{equation}

The noise eater reduces the heating rate by a factor of 10, which would translate to an increase in the lifetime from 0.56s to 5.8s, making the trap more usable for future applications. \\

\subsubsection{Heating Rate from Intensity Spectra}
As a further check to the validity of the model, we can also extract the heating rates directly from our intensity spectra. The relationship between heating rate along axis $ i $ and intensity noise is given by \cite{gehm1998dynamics}:

\begin{equation}
\Gamma_i=\pi^2\times f_{i}^2\times S_k(2f_{i})
\label{eq:gamma}
\end{equation}

where $S_k(2f_{i})$ is the one-sided power spectrum of the fractional fluctuation in the light intensity of the tweezer at twice the trap frequency of axis $ i $. Assuming ergodicity, the heating rate in the 3D trap is then given by the arithmetic average of the heating rate in each direction \cite{gehm1998dynamics}:

\begin{equation}
\Gamma=\frac{\Gamma_x+\Gamma_y+\Gamma_z}{3}
\label{eq:gamma_mean}
\end{equation}

To extract these heating rates, we measure our trap frequencies using Raman sideband spectroscopy\cite{PhysRevA.97.063423}. The trap frequencies in our cylindrical trap are:

\begin{equation}
\begin{split}
    f_{\text{radial}}&=f_x=f_y=\SI{360\pm 3}{\kilo \hertz}\\
    f_{\text{axial}}&=f_z=\SI{38\pm 1}{\kilo\hertz}\\
\end{split}
\label{eq:trap frequency}
\end{equation}

Using the noise spectra in figure \ref{fig:spectrum}, we extract the heating rates for the servo-ed and free running conditions:

\begin{equation}
    \begin{split}
        &\Gamma_{\text{free}} = \SI{5.1\pm0.9}{\second^{-1}}\\
        &\Gamma_{\text{servo}} = \SI{0.3\pm 0.1}{\second^{-1}}\\
    \end{split}
\end{equation}

These values are in reasonable agreement with the heating rates we extracted from the survival data (\ref{data_heating}), indicating that parametric heating is indeed the dominant mechanism limiting the trap lifetime. 



\begin{figure}[ht]
\centering
\includegraphics[width=12cm]{lifetime_MB.png}
\caption{The survival probability of the atom as a function of time. The blue and black points are the experimental data when the tweezer is servo-ed or free-running. The blue solid line and the black dashed line are the corresponding fits.}
\label{fig:lifetime}
\end{figure}



 Early approaches\cite{harb1994suppression, Taccheo:00} for intensity noise reduction directly fed back on the laser current, which is not possible for all laser systems, and focused on frequencies of up to 100 kHz. Another approach \cite{kwee2012stabilized} uses feedback on an acousto-optic modulator (AOM) for frequencies below 10 kHz and an optical cavity for mode cleanup for frequencies above 1 MHz. More recently, a light source with suppressed intensity noise\cite{blatt2015low} has been used for optical lattices to get stable trapping with long lifetimes. 
%(The requirements for the RIN may differ in both the required level and the frequency bands of interest across different applications.) 
Here, we present a general scheme for broadband noise reduction up to 1 MHz, independent of the laser source. It combines an electro-optic modulator (EOM) and an acousto-optic modulator (AOM) to independently deal with high ($\SI{100}{\kilo\hertz}$--$\SI{1}{\mega\hertz}$) and low (DC--$\SI{100}{\kilo\hertz}$) frequency intensity noise. We demonstrate our noise eater for use in an optical tweezer system. Lifetimes in optical tweezers are often limited by parametric heating\cite{gehm1998dynamics} at twice the trap frequency due to intensity noise. In optical tweezers, the typical trap frequencies are in the 10 kHz - 1 MHz region \cite{kaufman2012cooling, Liu900}, and we demonstrate up to 18 dB noise attenuation in this region. In particular, we improve our sodium atom lifetime in the optical tweezer from 0.56 s to 5.8s, making it utilizable for future experiments in coherent molecule production\cite{park2017second} or quantum gates\cite{ni2018dipolar}. 





%% OLD TEXT FROM 7/14/2020

% \caption{10 Hz - 300 kHz: - 3dB: 10 Hz, 0 dB: 70 Hz, 0 dB: 60 kHz, -3 dB: 300 kHz (about -0.5 dB at 100 kHz)
% 100 Hz - 1 MHz: -3dB: 100 Hz, 0 dB: 800 Hz, 0 dB: 700 kHz, - 3dB: 1 MHz 
% . { \bf{Low frequency:}} SRS 10 Hz to 300 kHz, digilent 100 (?) Hz to 100 kHz (?), used data 20 Hz to 100 kHz.  {\bf{High frequency:}} SRS 100 Hz to 1 MHz, digilent 1kHz to 1MHz, used data 50 kHz to 1MHz. \textcolor{red}{Why down to 30 Hz?  Is digilent range 100 Hz to 100 kHz?.  }}

% \begin{figure}[ht]
% \begin{subfigure}{.5\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=0.95\linewidth]{low_spec.png}  
%   \caption{High-frequency intensity noise spectrum}
%   \label{fig:high_spectrum}
% \end{subfigure}
% \begin{subfigure}{0.5\textwidth}
%   \centering
%   % include second image
%   \includegraphics[width=0.95\linewidth]{high_spect1.png}  
%   \caption{Low-frequency intensity noise spectrum}
%   \label{fig:low_spectrum}
% \end{subfigure}t

% \caption{\textcolor{blue}{Spectra without the Background}}
% \label{fig:spectrum}
% \end{figure}

% \begin{figure}[ht]
% \begin{subfigure}{.5\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=0.95\linewidth]{low_spect2.png}  
%   \caption{High-frequency intensity noise spectrum}
%   \label{fig:high_spectrum}
% \end{subfigure}
% \begin{subfigure}{0.5\textwidth}
%   \centering
%   % include second image
%   \includegraphics[width=0.95\linewidth]{high_spect2.png}  
%   \caption{Low-frequency intensity noise spectrum}
%   \label{fig:low_spectrum}
% \end{subfigure}

% \caption{\textcolor{blue}{Spectra with the same y range}}
% \label{fig:spectrum}
% \end{figure}




% \caption{\textcolor{blue}{}].
% The intensity noise spectrum. (a) Intensity noise spectrum in the high-frequency region. The yellow and the red curves shows the RIN with the noise eater off and on respectively. (b) Intensity noise spectrum in the low-frequency region. The red curve shows the RIN of the free-running laser. The yellow and purple curves show the RIN with the AOM servo off and on respectively, while keeping the EOM servo on. In both sub-figures, the background, due to the dark current of the photodetector, is shown in blue, and is well below the measured signals.}
% \label{fig:spectrum}
% \end{figure}




% \begin{figure}[ht]
% \centering
% \includegraphics[width=12cm]{high_spectrum.png}
% \caption{Intensity noise spectrum in the high frequency region from $\SI{50}{\kilo\hertz}$--$\SI{1}{\mega\hertz}$. The yellow and the red curves shows the RIN with the noise eater off and on respectively. The background, due to the dark current of the photodetector, is shown in blue, and is well below the measured signals.}
% \label{fig:high_spectrum}
% \end{figure}

% \begin{figure}[ht]
% \begin{subfigure}

% \centering
% \includegraphics[width=12cm]{low_spec_7_14.png}
% \caption{Intensity noise spectrum in the low-frequency region from $\SI{1}{\kilo\hertz}$(lower TODO)--$\SI{100}{\kilo\hertz}$. The blue curve shows the RIN of the free-running laser, without any servoing. The purple and red curves show the RIN with the AOM noise eater off and on respectively, while keeping the EOM noise eater on. The background, due to the dark current of the photodetector,  and is well below the measured signals.}
% \label{fig:low_spectrum}
% \end{subfigure}



% \begin{subfigure}[ht]{
% \centering
% \includegraphics[width=6cm]{suppression_negative.png}
% \caption{Noise reduction in the full frequency range. It is the intensity noise ratio of the free-running and servo-ed system. Twice our axial and radial trap frequencies are labeled for reference as the vertical lines.}
% \label{fig:suppresion}}
% \end{subfigure}
% \end{figure}
% \begin{figure}[ht]
% \centering
% \includegraphics[width=6cm]{suppression_negative.png}
% \caption{Noise reduction in the full frequency range. It is the intensity noise ratio of the free-running and servo-ed system. Twice our axial and radial trap frequencies are labeled for reference as the vertical lines.  \textcolor{red}{Decide which one you want. I prefer negative, but whatever. If you don't want to edit in inkscape or illustrator, then replot this with the python code and make look similar.  Instead of legend, put labels near the lines/vertical line. Using a legend is weird for a vertical line.}}
% \label{fig:suppresion}
% \end{figure}

%\begin{figure}[ht]
%\centering
%\includegraphics[width=12cm]{time_trace2.png}
%\caption{Experimental sequence for the lifetime test in the optical tweezer.}
%\label{fig:time}
%\end{figure}



% \begin{figure}[ht]
% \centering
% \begin{subfigure}[t]{.45\textwidth}
% \centering
%   % include first image
%   \parbox[][4cm][c]{.45\textwidth}{\includegraphics[width=0.9\linewidth]{lifetime_MB.png}}
%   \caption{The survival probability of the atom as a function of time. The blue and black points are the experimental data when the servo is active or not. The blue solid line and the black dashed line are the corresponding fits. }
%   \label{fig:lifetime}
% \end{subfigure}\hfil
% \begin{subfigure}[t]{0.45\textwidth}
% \centering
%   % include second image
% \includegraphics[width=\linewidth]{tweezer_figure_middled.png}
% \caption{Optical Tweezer Setup.The dotted rectangle shows the vacuum chamber. The red beam shows the Gaussian laser beam from the objective to trap the atom, which is shown with the white ball in the center. The trapped atom in the tweezer moves like a 3D harmonic oscillator with a low axial frequency and a high radial frequency.}
% \label{fig:lifetime}
% \end{subfigure}

% \end{figure}

==> Reduction of laser intensity noise over 1 MHz band for single atom trapping/Old/latexmkrc <==
## Sometimes when the references is very near the end of a page/column, latexmk fails to recognise when bibtex needs to be run. This rule forces bibtex to be run everytime.
$pdflatex = 'pdflatex --shell-escape %O %S; bibtex %R';



###############################
# Post processing of pdf file #
###############################

# assume the jobname is 'output' for Overleaf v2
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    my $QPDF = "/usr/bin/qpdf";
    return if ! -x $QPDF; # check that qpdf exists
    my $status = system($QPDF, "--linearize", "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
	system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
        $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
	system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
	if (-e $rtex_file) {
		do_knitr($rtex_file);
	}
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
	# change directory for a limited scope
	my $orig_dir = cwd();
	my $subdir = dirname($target);
	chdir($subdir);
	# run chktex on main file
	$status = system(
    "/usr/bin/run-chktex.sh",
    $orig_dir,
    $file
  );
	# go back to original directory
	chdir($orig_dir);

	# in VALIDATE mode we always exit after running chktex
	# otherwise we exit if EXIT_ON_ERROR is set

	if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
	    # chktex doesn't let us access the error info via exit status
	    # so look through the output
	    open(my $fh, "<", "output.chktex");
	    my $errors = 0;
	    {
		local $/ = "\n";
		while(<$fh>) {
		    if (/^\S+:\d+:\d+: Error:/) {
			$errors++;
			print;
		    }
		}
	    }
	    close($fh);
	    exit(1) if $errors > 0;
	    exit(0) if $ENV{'CHKTEX_VALIDATE'};
	}
    }
}

==> Reduction of laser intensity noise over 1 MHz band for single atom trapping/Old/scrap.tex <==
%\subsection{Draft Abstract, technique motivated}
%We developed a servo system with high-bandwidth intensity noise reduction for lasers. Up to $\SI{18}{\decibel}$ noise attenuation is achieved in the $\SI{100}{\kilo\hertz}$--$\SI{1}{\mega\hertz}$ region and the servo-ed laser provides us an optical tweezer where a single sodium atom has a lifetime of about 5 seconds, which is 10 times longer than the free-running condition. The stable, long-term trapping atoms could servo as a great platform for quantum computation and information. The servo design can be used for intensity noise reduction of any available wavelength and power, allowing coherent motional control of neural atoms, molecules and ions in general.
%\subsection{Draft Abstract, physics motivated}
%(maybe use in conclusion) Optical trapped neutral atoms and molecules have provided an attractive platform for quantum many-body physics, quantum information and computation. For those application, robust coherent quantum state is a crucial prerequisite. Coherent transfer is highly sensitive to the motional ground state occupancy of the individual atoms and requires long (> $\SI{1}{\second}$) trap lifetimes. Therefore, we developed a servo system which suppressed the intensity noise in a high bandwidth up to $\SI{1}{\mega\hertz}$, and obtained a stabilized optical trap where the trapped sodium atom has a lifetime of about 5 seconds.
% \textcolor{blue}{Eliot: I'm just writing random stuff to see what comes out}\\
%\textcolor{blue}{..................................................}\\

%For several decades, people have been using lasers. Lasers are great because they are stable both in frequency and intensity. There's a lot of applications for lasers, and most of them require some level of intensity stability, especially surrounding the frequencies relevant to the system of study. Some systems even require both DC control and low noise at frequencies higher than 100 kHz. Many lasers have integrated, internal noise eaters, but it can be helpful to have a general, external method for reducing noise when there are technological, practical, or financial limitations on the type of laser system you can buy.

%Our lab specifically uses lasers to form optical tweezers. Tweezers are super useful and have been demonstrated in several atomic species, and even molecular species (soon to be us!). However, to generalize tweezers for more species, we'll need stable light sources at a bunch of different frequencies. Furthermore, if you want an array of tweezers (as many labs do), you'll need a lot of power. This can prove limiting because it's possible there's not a clean, high-power laser source at the wavelength you need. 

%Our lab specifically is interested in developing an array of sodium tweezers for quantum chemistry and simulation reasons. Sodium tweezers need to be between 620 and 700 nm because of the AC Stark shift. However, we need like 3 W directly out of the laser per trap, and it's hard to find a direct laser source for that. We're therefore trying an SFG setup to produce the light. One of our input lasers happens to be noisy, which leads to noise on the output as well. The relevant requencies for our experiment is the shot-to-shot frequency (~3 Hz) and the parametric heating frequency (~500 kHz). Therefore, we need low noise at both DC (<10 Hz) and high frequency (200 kHz~1 MHz). This produces a major challenge, as we couldn't find any external noise eaters that work for DC-1 MHz.

%Our ingenious idea is to use two different servo systems to independently control high- and low- frequency noise.

%\textcolor{blue}{..................................................}\\
%\textcolor{blue}{Random stuff over}\\

%\textcolor{green}{~Something about lasers.~} 

%Lasers have become an important tool in a wide range of science and engineering fields due to their tight confinement of light and high frequency and intensity stability. 


%\textcolor{blue}{break}

%Optical tweezers have emerged as a powerful approach to a variety of applications in quantum simulation, quantum information, and quantum chemistry\cite{bernien2017probing,yu2019scalable,Liu900,PhysRevLett.120.113602} (pick better references). \textcolor{red}{I could add more general information here and put a paragraph break before moving on to our experiment} In our lab, we use tweezers to trap individual sodium and cesium atoms and combine them to coherently form NaCs molecules [cite]. Coherent transfer is highly sensitive to the motional ground state occupancy of the individual atoms and requires long (> $\SI{1}{\second}$) trap lifetimes. \textcolor{red}{Therefore, to achieve high transfer efficiency, we must limit heating of the atoms trapped in the tweezers}. The major heating mechanism in our system is parametric heating due to laser intensity fluctuations of the tweezer beams. Intensity noise at twice the harmonic trapping frequency is especially \textcolor{red}{damaging}, as it induces transitions between harmonic oscillator states in the trap \cite{PhysRevA.56.R1095}. For typical trap depths of a few $\si{\milli\kelvin}$, this means controlling intensity noise in the $\SI{100}{\kilo\hertz}$--$\SI{1}{\mega\hertz}$ band.


%   \cite{levine2019parallel,kaufman2012cooling}and .(TODO - maybe SNR?) of the experiments.....

 %However, most commercial laser noise eaters only work in a lower frequency region. Early approaches\cite{harb1994suppression, Taccheo:00} for intensity noise reduction directly fed back on the laser current, which is not possible for all laser drivers. More recently, a light source with suppressed intensity noise\cite{blatt2015low} has been used for optical lattices to get stable trapping with long lifetimes. 

%Here, we develop a servo system with high-bandwidth intensity noise reduction by combining an electro-optic modulator (EOM) servo and an acousto-optic modulator (AOM) servo to independently deal with high  ($\SI{100}{\kilo\hertz}$--$\SI{1}{\mega\hertz}$) and low (DC--$\SI{100}{\kilo\hertz}$) frequency noise. Up to $\SI{18}{\decibel}$ noise attenuation is achieved in the $\SI{100}{\kilo\hertz}$--$\SI{1}{\mega\hertz}$ region and up to $\SI{10}{\decibel}$ in the $1\si{\kilo\hertz}$--$\SI{100}{\kilo\hertz}$ region. With the servo system we developed, we can trap a single sodium atom for longer than $\SI{5}{\second}$, which provides a stable platform for various applications(TO cite). By suppressing parametric heating in our optical tweezer, we achieve a lifetime about 10 times longer than the free-running condition.(\textcolor{red}{if we find a pi, we will add a sentence here to show off our theory and experiment matches well}

%A fundamental prerequisite for laser sources suitable for optical dipole trapping is the occurrence \textcolor{blue}{(word choice)} of low relative intensity noise. Since the typical depth of optical dipole trap is a few $\si{\milli\kelvin}$ and the trap frequency is proportional to the square root of trap depth, the trap frequency is usually located in $100\si{\kilo}$--$\SI{1}{\mega\hertz}$, while commercial laser noise eater only works in a much lower frequency region(TODO). Due to the parametric heating mechanism, noise in this frequency region will greatly reduce the lifetime of an atom. This circumstance may strongly affect the lifetime of the atom trapped in the tweezer. This problem becomes a major constraint for quantum simulation or quantum computation applications which call for long coherence time.
%\textcolor{red}{An Eliot rewrite of the previous paragraph:}

%To get stable optical dipole traps with enough depth, 
%\textcolor{red}{experiment setup}

% \textcolor{blue}{.....................}
%  We generate $\SI{671}{\nano\meter}$ light with a sum-frequency generation (SFG) setup. We use a nonlinear crystal to combine $\SI{1557}{\nano\meter}$ light from an NKT photonics erbium-doped fiber laser with $\SI{1178}{\nano\meter}$ light from an MPB Raman fiber amplifier to get about $\SI{600}{\milli \watt}$ of $\SI{671}{\nano\meter}$ light. The intensity noise on the $\SI{671}{\nano\meter}$ light mainly comes from the $\SI{1178}{\nano\meter}$ laser and nonlinear effects of the crystal.
 
 %(VRFA-P-2000-589-SF)
 
 %\subsection{High-frequency servo}
%Our system setup is shown in Fig. \ref{fig:setup}. The $\SI{671}{\nano\meter}$ light exits the SFG crystal. We use a quarter waveplate and a half waveplate to modulate the polarization of the beam before entering the EOM so that about $80 \%$ the power transmits through the polarizing beam splitter (PBS). In this way, we get a balance of high power and best intensity noise reduction. We use a beam sampler to pick up about $1\%$ of the transmitted beam by the PBS after the EOM. One of the reflected beam from the sampler is for servoing and the other one is for monitoring. The beam for servoing is picked up by a $\SI{150}{\mega\hertz}$ bandwidth PDA10A photodiode and processed by a homemade proportional-integral-derivative (PID) circuit. A PDA36A photodiode with a bandwidth of $\SI{10}{\mega\hertz}$ bandwidth is used to monitor the noise spectrum. Both the feedback and monitoring photodiodes are placed on the transmission port of the PBS, as the reflection port has a different intensity noise spectrum.

% To maximize the noise reduction of the servo, the beam is focused by a plano-convex lens with a $\SI{75}{\milli\meter}$ focal length to the center of the active area of the servoing photodiode. In order to separate frequency regions, a bias tee is placed right after the photodiode so that the circuit only feeds back the high-frequency signal. The bias tee in our setup is homemade with a $\SI{3}{\decibel}$ attenuation cutoff at $\SI{17}{\kilo\hertz}$. It filters signals below the cutoff frequency without changing the phase or amplitude of the signal above the cutoff. Both the DC end of the bias tee and the setpoint of the PID circuit are terminated with standard $\SI{50}{\ohm}$ terminators. In the experiment, we use a combination of proportional and derivative control to minimize the noise in the high frequency region while keeping the bandwidth as large as possible. Since the maximum output signal of the PID circuit is relatively small, we add a homemade amplifier before the EOM to effectively increase the gain of the PID circuit. Two crucial points about the design of the amplifier are high gain and zero phase lag over a high bandwidth up to $\SI{1}{\mega\hertz}$. The high gain needs to match the halfwave voltage of the EOM so that the polarization of the light could be efficiently regulated. The zero phase lag will ensure the high bandwidth of the EOM servo. The open-loop transfer function of the PID together with the homemade amplifier is shown in Fig.\ref{fig:tf} for reference. It shows that in the high frequency region, it has a higher gain than in the low frequency region and a negative phase which effectively feed back to the loop.  

% Considered the phase delay in EOM and the optical path, the EOM servo system is a controlled object with inertia, and we need to improve the dynamic characteristics of the system adjustment process. \textcolor{red}{(This previous sentence is confusing. Not really sure what you mean here.)} In order to avoid the possible oscillation and even destabilization during the adjustment of the error, we want to have a phase-lead compensator, which is generated by a combination of proportional and derivative feedback. The circuit we are using have two proportional control, two integral control and one derivative control. \textcolor{red}{We should talk about this paragraph.}
 
 
%\textcolor{red}{*}After the circuit, we add another homemade electric amplifier to the output of the servo and connect it to the EOM. 
%The main idea of the design of the amplifier is to match the maximum noise signal with the voltage required to produce a retardant of $\pi$ rad with a broad bandwidth. \textcolor{red}{This sentence is confusing.} The combination of the waveplate configuration is carefully designed to make sure the EOM could act on the slope of the polarization while wasting less optical power. The amplitude modulating EOM operates as a voltage dependent waveplate. There are a fast and a slow axis in the birefringent crystal whose birefringence depends on the applied voltage. It introduces a phase delay between the two axes. 

% To measure the spectra, we use a low-noise SR560 preamplifier from Stanford Research Systems to improve the signal-to-noise ratio (SNR) and measure it with a Digital Discovery field programmable gate array (FPGA) board from Digilent. The $\SI{1}{\mega\hertz}$ bandwidth of the preamplifier covers the frequency region we are interested in. Additionally, we measure the spectra above $\SI{1}{\mega\hertz}$ using a ZFL-1000LN+ amplifier from Mini-circuits. The results show that the EOM servo has no appreciable effect on the intensity noise spectrum up to $\SI{10}{\mega\hertz}$. since the SR560 preamplifier has a flatter gain in a large range which makes the measurement convenient, all spectra presented in this paper are measured with the Stanford Research Systems preamplifier.

% In Fig. \ref{fig:high_spectrum}, we show the comparison of the intensity noise spectral densities with and without the servo. The spectra are normalized to the DC power and are commonly
% referred to as relative intensity-noise (RIN) spectra. These spectra are measured on the experiment table before the vacuum chamber so that the noise of the fiber is also considered. The background is measured when the light is blocked so it is mainly caused by the dark current of the photodiode. The spectra are normalized to the DC power and are commonly referred to as relative intensity-noise (RIN) spectra \textcolor{blue}{cite}. The intensity noise is reduced by up to $\SI{18}{\decibel}$ for Fourier frequencies below $\SI{1}{\mega\hertz}$. Though the intensity noise of the free-running laser is not evenly distributed over the high-frequency region, it is almost constant when servoed, allowing stable trapping with long lifetimes in different trap depths.

% \subsection{AOM servo}
%After the EOM servo, we use an AOM servo to control the low frequencies from DC to about $\SI{100}{\kilo\hertz}$. We focus the beam into the AOM to maximize its switching bandwidth. The beam of the first diffraction order is re-collimated by another plano-convex lens with the same focal length while the zeroth order is dumped (which is not shown in the Fig.\ref{fig:setup}). The signal for the servo is picked up by a wedged beam sampler and focused onto a PDA10A2 photodiode. Here, we use the same model bias tee as in the high-frequency servo to filter out the high frequency noise. The bandwidth of the DC (low-pass) end is about $\SI{100}{\kilo\hertz}$ and the RF end is terminated with a standard $\SI{50}{\ohm}$ terminator. The DC output of the bias tee is connected to the input of the PID circuit and the DC setpoint of the PID is controlled by the experiment control computer. To reduce the steady-state error and stabilize the servo, we primarily use integral control with little proportional or derivative feedback. A $\SI{100}{\kilo\hertz}$ low-pass filter is added to the output of the circuit to ensure that no high-frequency electronic noise is written onto the optical intensity spectrum. We tune the PID settings so that the PID does not introduce any other resonance, especially in the high frequency region. The RF signal for driving the AOM is combined with the servo signal with the mixer ZAD-1-1+ . We set the RF signal amplitude such that the AOM transmission reaches maximum when the servo is railed. In the experiment, we change the DC power of the light by changing the setpoint of the servo, which effectively changes the RF power driving the AOM.

% The AOM servo provides DC power control and an up to $\SI{10}{\decibel}$ intensity noise suppression in a lower frequency region, as shown in Fig. \ref{fig:low_spectrum}. We measure the intensity noise spectrum when the laser is blocked (background), free-running, only EOM servo-ed (with AOM servo railed), and both AOM and EOM servo-ed. It is clear that the EOM servo doesn't add extra noise in the low frequency region and the AOM servo only slightly increases noise in the intermediate region from $\SI{10}{\kilo\hertz}$ to $\SI{100}{\kilo\hertz}$. It could be re-optimized for better performance if required and also there are commercial products dealing with this frequency region.

% Based on the spectra in the high and low frequency regions, we calculate the suppression factor of our servo system in the full frequency band in Fig.\ref{fig:suppresion}. For reference, we also label approximately twice our axial and radial trapping frequencies in the figure. From the suppression factor figure, we see an approximately $\SI{2}{\decibel}$ intensity noise reduction at twice the axial frequency and an $\SI{13}{\decibel}$reduction at twice the radial frequency of our optical tweezer.

% The $\SI{1}{\mega\hertz}$ bandwidth of the preamplifier covers the frequency region we are interested in. Additionally, we measure the spectra above $\SI{1}{\mega\hertz}$ using a ZFL-1000LN+ amplifier from Mini-circuits.
%The results show that the EOM servo has no appreciable effect on the intensity noise spectrum up to $\SI{10}{\mega\hertz}$.

. For a set of given parameter including the initial temperature and the heating rate, we could numerically solve the Fokker Planck equation and get the survival probability as a function of time. The $\chi^2$ is defined by the square of the error between the experimental data and the calculated survival probability divided by the uncertainty in the experiment:

\textcolor{blue}{..................................................}
We characterize the effect of tweezer intensity noise on the atom by measuring trap lifetimes under different servo conditions. A time plot of the experimental sequence is shown in Fig. \ref{fig:time}. Due to technical reasons (\textcolor{blue}{limited power}), we are unable to load atoms directly into our $\SI{671}{\nano\meter}$ tweezer. Instead, we load and image atoms first in a $\SI{700}{\nano\meter}$ tweezer, then transfer to the $\SI{671}{\nano\meter}$ tweezer. We then transfer back to the $\SI{700}{\nano\meter}$ tweezer for final atomic imaging. We measured the trap depth and trap frequency of the $\SI{700}{\nano\meter}$ tweezer by Raman sideband spectrum and rescale the complex polarizability for $\SI{671}{\nano\meter}$\cite{grimm2000optical}. The trap depth $U_0$ and the effective trap frequency $f_{trap}$ are: 
\begin{equation}
    \begin{split}
        U_0&=\SI{5.7}{\milli\kelvin} \\
        f_{trap}&=\SI{295}{\kilo\hertz}
    \end{split}
\end{equation}

By varying the hold time of the tweezer and observing how the survival probability varies with time, we can extract the heating rate. Lifetime measurements for the two servo conditions are shown in Fig. \ref{fig:lifetime}. For every data point, we load over 500 atoms. We find exceptionally low heating rates and correspondingly long lifetimes when the tweezer light is controlled by our intensity noise reduction system.

%\textcolor{brown}{present the extracted heating rate and compare it to the noise intensity}
We fit the survival probabilities to a curve following the procedure in \cite{gehm1998dynamics}. We assume an initial Maxwell-Boltzmann energy probability density with the temperature as a free fitting parameter since every single test we load only one atom in the tweezer and there is no exchange interaction. For a set of given parameter including the initial temperature and the heating rate, we could numerically solve the Fokker Planck equation and get the survival probability as a function of time. The $\chi^2$ is defined by the square of the error between the experimental data and the calculated survival probability divided by the uncertainty in the experiment:
\begin{equation}
    \chi^2(T_0, \Gamma_{1}, \Gamma_{2})=\sum_{i=1,2...5}\frac{(x_{1_i}-x(t_i, T_0, \Gamma_1))^2}{{\sigma_1}_i^2} + \sum_{j=1,2...7}\frac{({x_2}_j- x({t_2}_j, T_0, \Gamma_2))^2}{{\sigma_2}_j^2}
\end{equation}
The subscript 1 refers to the free-running condition and 2 for with the servo. $\Gamma_{1,2}$ is the heating rate and $T_0$ is the initial temperature of the atoms in the tweezer. The time series we measure the survival probability is donated by $t_{1,2}$, the corresponding survival probabilities are donated by $x_{1,2}$ and the uncertainty by $\sigma_{1,2}$. $x(t,T,\Gamma)$ is survival probability calculated by the numerical integral of density distribution below the trap depth where the density distribution is the numerical solution of the Fokker-Planck equation at the time $t$ with the heating rate $\Gamma$ and initial temperature $T$. The optimization process is to find a set of proper $\Gamma_{1,2}$,$T_0$ so that the $\chi^2$ is minimized. We do the optimization by a two level scan: firstly we fix the $T_0$ and scan $\Gamma_1$ and $\Gamma_2$, as the two summation terms are independent(first summation only relies on $\Gamma_1$ and the second summation only relies on $\Gamma_2$), we separately scan $\Gamma_1$ and scan $\Gamma_2$ to find a minimized $\chi^2$ with the fixed $T_0$; secondly we scan the $T_0$ to minimize $\chi^2$. We then find the global minimum of $\chi^2$ and take the corresponding parameter as the fitting results.
%We then optimize the fit of each curve by varying the heating rates. The time evolution of the distribution is described by the Fokker-Plank equation. The survival probabilities are calculated by the summation of the atoms with less energy than the trap depth. 
From the fitted curves, we calculate the initial temperature and heating rates of the system to be:
\begin{equation}
    \begin{split}
        &T_0 = \SI{0.50\pm0.02}{\milli\kelvin}\\
        &\Gamma_{1} = \SI{3.50\pm 0.03}{\second^{-1}}\\
        &\Gamma_{2} = \SI{0.348\pm 0.003}{\second^{-1}}\\
    \end{split}
\end{equation}

%where the heating rate $\Gamma$ is defined as the exponential growth rate of the average energy: 
%\begin{equation}
%    \langle \dot{E} \rangle=\Gamma E
%\end{equation}

From the relationship between heating rate and intensity noise,
\begin{equation}
\Gamma_x=\pi^2\times f_{x}^2\times S_k(2f_{tx})
\label{eq:gamma}
\end{equation}
where $S_k(2f_{x})$ is the one-sided power spectrum of the fractional fluctuation in the spring constant of the tweezer at double trap frequency in x dimension. And the effective heating rate of this system is the arithmetic mean of the heating rate of the three dimensions:

\begin{equation}
\Gamma=\frac{\Gamma_x+\Gamma_y+\Gamma_z}{3}
\label{eq:gamma_mean}
\end{equation}

In our system, we measured the trap frequency in three dimensions by TODO and got
\begin{equation}
\begin{split}
    f_{\text{radial}}&=f_x=f_y=\SI{360\pm 3}{\kilo \hertz}\\
    f_{\text{axial}}&=f_z=\SI{38\pm 1}{\kilo\hertz}\\
\end{split}
\label{eq:trap frequency}
\end{equation}
we measured the experimental heating rate for both condition(the subscribe n refers to results calculated by noise spectra):
\begin{equation}
    \begin{split}
     &\Gamma_{\text{free}} = \SI{5.1\pm0.9}{\second^{-1}}\\
     &\Gamma_{\text{servo}} = \SI{0.3\pm 0.1}{\second^{-1}}\\
    \end{split}
\end{equation}
The noise spectra results and the lifetime test on the atom are in close agreement that 10 times lifetime of the atom in the tweezer is gained by the servo system and the half-life of the sodium atom is longer than $\SI{5}{\second}$.  

We stochastically load sodium atoms from a magneto-optical trap (MOT) \cite{hutzler2017eliminating}. After turning off the MOT, we image the atoms in a 700 nm trap, in order to then post select on trials where a sodium atom is successfully loaded. We then transfer the atom to the 671 nm trap, in the servo-ed and free running condition for variable hold times. We then image again, back in the 700 nm trap, to see if the atom had been lost from the trap. The survival probability of the atom as a function of time is shown in figure \ref{fig:lifetime}. There is a clear increase in the atom lifetime when the noise eater system is used. \\

\subsection{Quantitative Analysis}
To confirm that parametric heating is indeed the mechanism for atom loss, we take a more quantitative approach. We extract heating rates from the survival data in figure \ref{fig:liftime}. Furthermore, we also compare these heating rates to the expected heating rates based on the measured intensity noise spectrum of the laser. 

\subsubsection{Heating Rate from Atom Survival}
We fit the survival probabilities following the model in \cite{gehm1998dynamics}. We assume an initial Maxwell-Boltzmann energy distribution, instead of a Bose-Einstein distribution, since we are loading atoms one at a time. We then evolve the energy distribution to time $ t $ using a Fokker-Planck equation with a heating rate, $ \Gamma $. Then, to obtain the survival of the atoms, we calculate the portion of the distribution that is lower in energy than the trap depth. From this procedure, we fit the heating rate, and the ratio of the initial temperature to the trap depth. We measure the trap power, beam waist, and convert to a trap depth using the polarizability \cite{arora2007magic}. Using this trap depth of 5.7 mK, we can then extract an initial temperature, $ T_0 $. \\
We fit both the servo-ed and free running cases shown in figure \ref{fig:lifetime} together, extracting a common $T_0$ along with heating rates, $\Gamma_{\text{servo}}$ and $ \Gamma_{\text{free}} $:

\begin{equation} \label{data_heating}
    \begin{split}
        &T_0 = \SI{0.50\pm0.02}{\milli\kelvin}\\
        &\Gamma_{\text{free}} = \SI{3.50\pm 0.03}{\second^{-1}}\\
        &\Gamma_{\text{servo}} = \SI{0.348\pm 0.003}{\second^{-1}}\\
    \end{split}
\end{equation}

The noise eater reduces the heating rate by a factor of 10, which would translate to an increase in the lifetime from 0.56s to 5.8s, making the trap more usable for future applications. \\

\subsubsection{Heating Rate from Intensity Spectra}
As a further check to the validity of the model, we can also extract the heating rates directly from our intensity spectra. The relationship between heating rate along axis $ i $ and intensity noise is given by \cite{gehm1998dynamics}:

\begin{equation}
\Gamma_i=\pi^2\times f_{i}^2\times S_k(2f_{i})
\label{eq:gamma}
\end{equation}

where $S_k(2f_{i})$ is the one-sided power spectrum of the fractional fluctuation in the light intensity of the tweezer at twice the trap frequency of axis $ i $. Assuming ergodicity, the heating rate in the 3D trap is then given by the arithmetic average of the heating rate in each direction \cite{gehm1998dynamics}:

\begin{equation}
\Gamma=\frac{\Gamma_x+\Gamma_y+\Gamma_z}{3}
\label{eq:gamma_mean}
\end{equation}

To extract these heating rates, we measure our trap frequencies using Raman sideband spectroscopy\cite{PhysRevA.97.063423}. The trap frequencies in our cylindrical trap are:

\begin{equation}
\begin{split}
    f_{\text{radial}}&=f_x=f_y=\SI{360\pm 3}{\kilo \hertz}\\
    f_{\text{axial}}&=f_z=\SI{38\pm 1}{\kilo\hertz}\\
\end{split}
\label{eq:trap frequency}
\end{equation}

Using the noise spectra in figure \ref{fig:spectrum}, we extract the heating rates for the servo-ed and free running conditions:

\begin{equation}
    \begin{split}
        &\Gamma_{\text{free}} = \SI{5.1\pm0.9}{\second^{-1}}\\
        &\Gamma_{\text{servo}} = \SI{0.3\pm 0.1}{\second^{-1}}\\
    \end{split}
\end{equation}

These values are in reasonable agreement with the heating rates we extracted from the survival data (\ref{data_heating}), indicating that parametric heating is indeed the dominant mechanism limiting the trap lifetime. 



\begin{figure}[ht]
\centering
\includegraphics[width=12cm]{lifetime_MB.png}
\caption{The survival probability of the atom as a function of time. The blue and black points are the experimental data when the tweezer is servo-ed or free-running. The blue solid line and the black dashed line are the corresponding fits.}
\label{fig:lifetime}
\end{figure}



 Early approaches\cite{harb1994suppression, Taccheo:00} for intensity noise reduction directly fed back on the laser current, which is not possible for all laser systems, and focused on frequencies of up to 100 kHz. Another approach \cite{kwee2012stabilized} uses feedback on an acousto-optic modulator (AOM) for frequencies below 10 kHz and an optical cavity for mode cleanup for frequencies above 1 MHz. More recently, a light source with suppressed intensity noise\cite{blatt2015low} has been used for optical lattices to get stable trapping with long lifetimes. 
%(The requirements for the RIN may differ in both the required level and the frequency bands of interest across different applications.) 
Here, we present a general scheme for broadband noise reduction up to 1 MHz, independent of the laser source. It combines an electro-optic modulator (EOM) and an acousto-optic modulator (AOM) to independently deal with high ($\SI{100}{\kilo\hertz}$--$\SI{1}{\mega\hertz}$) and low (DC--$\SI{100}{\kilo\hertz}$) frequency intensity noise. We demonstrate our noise eater for use in an optical tweezer system. Lifetimes in optical tweezers are often limited by parametric heating\cite{gehm1998dynamics} at twice the trap frequency due to intensity noise. In optical tweezers, the typical trap frequencies are in the 10 kHz - 1 MHz region \cite{kaufman2012cooling, Liu900}, and we demonstrate up to 18 dB noise attenuation in this region. In particular, we improve our sodium atom lifetime in the optical tweezer from 0.56 s to 5.8s, making it utilizable for future experiments in coherent molecule production\cite{park2017second} or quantum gates\cite{ni2018dipolar}. 





%% OLD TEXT FROM 7/14/2020

% \caption{10 Hz - 300 kHz: - 3dB: 10 Hz, 0 dB: 70 Hz, 0 dB: 60 kHz, -3 dB: 300 kHz (about -0.5 dB at 100 kHz)
% 100 Hz - 1 MHz: -3dB: 100 Hz, 0 dB: 800 Hz, 0 dB: 700 kHz, - 3dB: 1 MHz 
% . { \bf{Low frequency:}} SRS 10 Hz to 300 kHz, digilent 100 (?) Hz to 100 kHz (?), used data 20 Hz to 100 kHz.  {\bf{High frequency:}} SRS 100 Hz to 1 MHz, digilent 1kHz to 1MHz, used data 50 kHz to 1MHz. \textcolor{red}{Why down to 30 Hz?  Is digilent range 100 Hz to 100 kHz?.  }}

% \begin{figure}[ht]
% \begin{subfigure}{.5\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=0.95\linewidth]{low_spec.png}  
%   \caption{High-frequency intensity noise spectrum}
%   \label{fig:high_spectrum}
% \end{subfigure}
% \begin{subfigure}{0.5\textwidth}
%   \centering
%   % include second image
%   \includegraphics[width=0.95\linewidth]{high_spect1.png}  
%   \caption{Low-frequency intensity noise spectrum}
%   \label{fig:low_spectrum}
% \end{subfigure}t

% \caption{\textcolor{blue}{Spectra without the Background}}
% \label{fig:spectrum}
% \end{figure}

% \begin{figure}[ht]
% \begin{subfigure}{.5\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=0.95\linewidth]{low_spect2.png}  
%   \caption{High-frequency intensity noise spectrum}
%   \label{fig:high_spectrum}
% \end{subfigure}
% \begin{subfigure}{0.5\textwidth}
%   \centering
%   % include second image
%   \includegraphics[width=0.95\linewidth]{high_spect2.png}  
%   \caption{Low-frequency intensity noise spectrum}
%   \label{fig:low_spectrum}
% \end{subfigure}

% \caption{\textcolor{blue}{Spectra with the same y range}}
% \label{fig:spectrum}
% \end{figure}




% \caption{\textcolor{blue}{}].
% The intensity noise spectrum. (a) Intensity noise spectrum in the high-frequency region. The yellow and the red curves shows the RIN with the noise eater off and on respectively. (b) Intensity noise spectrum in the low-frequency region. The red curve shows the RIN of the free-running laser. The yellow and purple curves show the RIN with the AOM servo off and on respectively, while keeping the EOM servo on. In both sub-figures, the background, due to the dark current of the photodetector, is shown in blue, and is well below the measured signals.}
% \label{fig:spectrum}
% \end{figure}




% \begin{figure}[ht]
% \centering
% \includegraphics[width=12cm]{high_spectrum.png}
% \caption{Intensity noise spectrum in the high frequency region from $\SI{50}{\kilo\hertz}$--$\SI{1}{\mega\hertz}$. The yellow and the red curves shows the RIN with the noise eater off and on respectively. The background, due to the dark current of the photodetector, is shown in blue, and is well below the measured signals.}
% \label{fig:high_spectrum}
% \end{figure}

% \begin{figure}[ht]
% \begin{subfigure}

% \centering
% \includegraphics[width=12cm]{low_spec_7_14.png}
% \caption{Intensity noise spectrum in the low-frequency region from $\SI{1}{\kilo\hertz}$(lower TODO)--$\SI{100}{\kilo\hertz}$. The blue curve shows the RIN of the free-running laser, without any servoing. The purple and red curves show the RIN with the AOM noise eater off and on respectively, while keeping the EOM noise eater on. The background, due to the dark current of the photodetector,  and is well below the measured signals.}
% \label{fig:low_spectrum}
% \end{subfigure}



% \begin{subfigure}[ht]{
% \centering
% \includegraphics[width=6cm]{suppression_negative.png}
% \caption{Noise reduction in the full frequency range. It is the intensity noise ratio of the free-running and servo-ed system. Twice our axial and radial trap frequencies are labeled for reference as the vertical lines.}
% \label{fig:suppresion}}
% \end{subfigure}
% \end{figure}
% \begin{figure}[ht]
% \centering
% \includegraphics[width=6cm]{suppression_negative.png}
% \caption{Noise reduction in the full frequency range. It is the intensity noise ratio of the free-running and servo-ed system. Twice our axial and radial trap frequencies are labeled for reference as the vertical lines.  \textcolor{red}{Decide which one you want. I prefer negative, but whatever. If you don't want to edit in inkscape or illustrator, then replot this with the python code and make look similar.  Instead of legend, put labels near the lines/vertical line. Using a legend is weird for a vertical line.}}
% \label{fig:suppresion}
% \end{figure}

%\begin{figure}[ht]
%\centering
%\includegraphics[width=12cm]{time_trace2.png}
%\caption{Experimental sequence for the lifetime test in the optical tweezer.}
%\label{fig:time}
%\end{figure}



% \begin{figure}[ht]
% \centering
% \begin{subfigure}[t]{.45\textwidth}
% \centering
%   % include first image
%   \parbox[][4cm][c]{.45\textwidth}{\includegraphics[width=0.9\linewidth]{lifetime_MB.png}}
%   \caption{The survival probability of the atom as a function of time. The blue and black points are the experimental data when the servo is active or not. The blue solid line and the black dashed line are the corresponding fits. }
%   \label{fig:lifetime}
% \end{subfigure}\hfil
% \begin{subfigure}[t]{0.45\textwidth}
% \centering
%   % include second image
% \includegraphics[width=\linewidth]{tweezer_figure_middled.png}
% \caption{Optical Tweezer Setup.The dotted rectangle shows the vacuum chamber. The red beam shows the Gaussian laser beam from the objective to trap the atom, which is shown with the white ball in the center. The trapped atom in the tweezer moves like a 3D harmonic oscillator with a low axial frequency and a high radial frequency.}
% \label{fig:lifetime}
% \end{subfigure}

% \end{figure}
